Thompson Sampling Achieves $\tilde O(\sqrt{T})$ Regret in Linear Quadratic Control

Thompson Sampling (TS) is an efficient method for decision-making under uncertainty, where an action is sampled from a carefully prescribed distribution which is updated based on the observed data. In this work, we study the problem of adaptive control of stabilizable linear-quadratic regulators (LQRs) using TS, where the system dynamics are unknown. Previous works have established that $\tilde O(\sqrt{T})$ frequentist regret is optimal for the adaptive control of LQRs. However, the existing methods either work only in restrictive settings, require a priori known stabilizing controllers, or utilize computationally intractable approaches. We propose an efficient TS algorithm for the adaptive control of LQRs, TS-based Adaptive Control, TSAC, that attains $\tilde O(\sqrt{T})$ regret, even for multidimensional systems, thereby solving the open problem posed in Abeille and Lazaric (2018). TSAC does not require a priori known stabilizing controller and achieves fast stabilization of the underlying system by effectively exploring the environment in the early stages. Our result hinges on developing a novel lower bound on the probability that the TS provides an optimistic sample. By carefully prescribing an early exploration strategy and a policy update rule, we show that TS achieves order-optimal regret in adaptive control of multidimensional stabilizable LQRs. We empirically demonstrate the performance and the efficiency of TSAC in several adaptive control tasks.

==> sections/prior_ts.tex <==
In \cite{abeille2018improved}, the authors propose a TS algorithm for adaptive control of an unknown LQR. At each time step $t$, given $\hat{\Theta}_t$, their algorithm samples a perturbed parameter $\Tilde{\Theta}_t$ until the sampled parameter belongs to their admissible set, $\Bar{\mathcal{S}}$. This operation is denoted as $\mathcal{R}_{\Bar{\mathcal{S}}}(\hat{\Theta}_t + \beta_t(\delta) V_{t}^{-1/2} \eta_t )$ where $\eta_t \in \mathbb{R}^{(n+d)\times n}$ is the perturbation matrix which has component-wise normal distribution. The random sampling is achieved coherently with regularized least squares estimation and the uncertainty within $V_t$. Here $\mathcal{R}_{\Bar{\mathcal{S}}}$ denotes the rejection sampling to guarantee that the randomly sampled parameter is within their admissible set $\Bar{\mathcal{S}}$. However, their admissible set only includes ``contractible'' systems:
\begin{equation*}
    \Bar{\mathcal{S}} = \{ \Bar{\Theta} ~\big|~ J(\Bar{\Theta}) \leq D, \|\Bar{A} - \Bar{B} K(\Bar{\Theta}) \| < 1,  \|\Bar{\Theta}\|_F \leq S\}.
\end{equation*}

This set is a subset of the set defined in Assumption \ref{admissible_set}, since for any stabilizable system there exists a similarity transformation that makes the underlying system contractible. Notice that these sets are equivalent to each other when the underlying system is scalar since $\rho(A_* - B_* K(\Theta_*)) = \|A_* - B_* K(\Theta_*) \|_2$ for any scalar system $\Theta_*$. In \cite{abeille2018improved}, the authors show that this sampling strategy provides samples that are concentrated around $\hat{\Theta}$ which in turn are concentrated around $\Theta_*$, yielding a bounded state throughout the TS based adaptive control. In the following section, we first study an only TS-based adaptive control algorithm in multi-dimensional LQRs. 

